Multi-Cue Vehicle Detection for Semantic Video Compression In Georegistered Aerial Videos

Detection of moving objects such as vehicles in videos acquired from an airborne camera is very useful for video analytics applications. Using fast low power algorithms for onboard moving object detection would also provide region of interest-based semantic information for scene content aware image compression. This would enable more efficient and flexible communication link utilization in lowbandwidth airborne cloud computing networks. Despite recent advances in both UAV or drone platforms and imaging sensor technologies, vehicle detection from aerial video remains challenging due to small object sizes, platform motion and camera jitter, obscurations, scene complexity and degraded imaging conditions. This paper proposes an efficient moving vehicle detection pipeline which synergistically fuses both appearance and motion-based detections in a complementary manner using deep learning combined with flux tensor spatio-temporal filtering. Our proposed multi-cue pipeline is able to detect moving vehicles with high precision and recall, while filtering out false positives such as parked vehicles, through intelligent fusion. Experimental results show that incorporating contextual information of moving vehicles enables high semantic compression ratios of over 100:1 with high image fidelity, for better utilization of limited bandwidth air-to-ground network links.

==> TXT/02_video_stablization.tex <==
\section{Assistive Tasks}

This section describes the tasks and methods that are essential and applied in our processing pipeline, however they are not the main focus of the paper. 



\begin{figure*}[t!]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.98\linewidth]{Figs/results.PNG}
\end{center}
   \caption{Intermediate results and the final result after applying the pipeline. a) Raw data, b) Motion mask $M_{M_t}$ overlaid on flux tensor motion based detection. c) Appearance mask $M_{M_t}$ overlaid on the raw frame, the red overlaid masks represent all predicted vehicles(moved and parked) in the scene. d) Appearance-motion fusion result, some false positive appears on the top of the buildings. e) Buildings mask $M_{P_t}$. f) The final result after filter out false positives on the top of the building.} 
\label{fig:results}
\end{figure*}

==> TXT/04_applications.tex <==
\subsection{Post detection analysis}
%-------------------------------------
\begin{figure*}[h!]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.95\linewidth]{Figs/MOT.PNG}
\end{center}
   \caption{Multi-object tracking implementation on moving vehicles detection}
\label{fig:MOT}
\end{figure*}

Object detection is the first step on many advance computer vision applications (e.g. Muli-object tracking~\cite{al2017robust,al2018multi}, video summarization~\cite{ekin2003automatic, lee2012discovering}, and behaviour understanding~\cite{adam2008robust}.
\subsubsection{Muli-object tracking}
Since the rapid progress in object detection techniques \cite{girshick2015fast,palaniappan2007moving,girshick2014rich}, tracking-by-detection \cite{andriluka2008people,breitenstein2011online,al2017robust,al2018multi} becomes popular among multi-object tracking approaches. In this paper, our multi-object tracker is used to extend the results obtained form object detection as a case study. The tracker is detection-based that uses a two-step data association scheme to ensure high tracking accuracy and continuity. The first step ensures having reliable short-term tracklets using only spatial information. The second step links tracklets globally and reduces matching hypotheses using discriminative features(e.g histogram of gradient (HoG), color, and tracklets history). Figure~\ref{fig:MOT} shows the trajectories for the predicted results.
%--------------------
\subsection{Video summarization }
Recently, the demand for online and real time applications that required video data has been increased dramatically~\cite{hanisch2003modeling,ezaki2012pedestrian}. Efficient handling of video information is important to ensure optimum storage capacity, smoother videos transmission, fast and reliable video processing. Video summarization is the process of generating an abstract from videos to be used for storage or retrieval system. For our case, video summarization is used for system retrieving. The first frame from the video will be sent to destination cite followed by a abstract frames that have only the predicted vehicles. This technique reduces transfer cost to 66:1. Figure~\ref{fig:summer} shows the entire process for video transmission from source to destination cite. The cost of transferring raw data versus the abstracted ones described~\ref{table:commpression}
% %-------------------------------------------
% \begin{table}[b]
% \scalebox{0.88}{
% \caption{Data transfer cost.}
% \label{table:commpression}
% \begin{tabular}{|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{Type}      & \multicolumn{1}{c|}{Size}   & \multicolumn{1}{c|}{Compression ratio} \\ \hline
% \hline
% 200 x Raw RGB                                                                & 1070 MB                                                                     & \multirow{3}{$\times$}{66 times}             \\ 
% \cline{1-2}
% \begin{tabular}[c]{@{}l@{}}1 Raw \\ 199 masked/ abstract frames\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}6 MB\\ 10.3 MB\end{tabular}} &                                        \\ \cline{1-2}
% Total                                                                        & 16.3 MB                                                                     &                                        \\ \hline
% \end{tabular}
% }
% \end{table}
% %-------------------------------------------
\begin{table}[t!]
\caption{Data transfer cost. Raw corresponds to original RGB video frame. Masked image is obtained by keeping the RGB values for detection regions and setting background pixels to zero. In the proposed cases, first frame in the sequence is transferred as a raw frame to encode general scene structures. For the remaining frames, masked frames encoding only the detected objects are transferred, greatly reducing the data transfer costs.}
\label{table:commpression}
\scalebox{0.89}{
\begin{center}
\begin{tabular}{|l|l|r|p{0.5in}|}
\hline
Detection Method  & Image Type &  Data Size  & Compress. \\
\hline
\hline
Raw video & 200 $\times$ Raw &  1070 MB & $\times$ 1\\
\hline
Motion (Flux tensor) & 1 $\times$ Raw  & 6 MB & $\times$ 41\\
              
            & 199 $\times$ Masked  &  26 MB & \\
\hline
Appearance(YOLO) & 1 $\times$ Raw  & 6 MB & $\times$ 35 \\
              
            & 199 $\times$ Masked  &  30 MB & \\
\hline
Flux + YOLO & 1 $\times$ Raw  & 6 MB & $\times$ 56 \\
            & 199 $\times$ Masked  & 19 MB  & \\
\hline
Flux + YOLO  & 1 $\times$ Raw  & 6 MB & \\ 
+ Building   & 199 $\times$ Masked  & 10.3 MB &  $\times$ 66\\ 
\hline
\end{tabular}
\end{center}
}
\end{table}
% %-------------------------------------------
% \begin{table}[b]
% \scalebox{0.88}{
% \caption{Data transfer cost.}
% \label{table:commpression}
% \begin{tabular}{|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{Type}      & \multicolumn{1}{c|}{Size}   & \multicolumn{1}{c|}{Compression ratio} \\ \hline
% \hline
% 200 x Raw RGB                                                                & 1070 MB                                                                     & \multirow{3}{$\times$}{66 times}             \\ 
% \cline{1-2}
% \begin{tabular}[c]{@{}l@{}}1 Raw \\ 199 masked/ abstract frames\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}6 MB\\ 10.3 MB\end{tabular}} &                                        \\ \cline{1-2}
% Total                                                                        & 16.3 MB                                                                     &                                        \\ \hline
% \end{tabular}
% }
% \end{table}
% %-------------------------------------------

\begin{figure*}[h!]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=1\linewidth]{Figs/summer.PNG}
\end{center}
   \caption{Transferring procedure between source and destination cites.}
\label{fig:summer}
\end{figure*}
